Safe and Stabilizing Distributed Multi-Path Cellular Flows

We study the problem of distributed traffic control in the partitioned plane, where the movement of all entities (robots, vehicles, etc.) within each partition (cell) is coupled. Establishing liveness in such systems is challenging, but such analysis will be necessary to apply such distributed traffic control algorithms in applications like coordinating robot swarms and the intelligent highway system. We present a formal model of a distributed traffic control protocol that guarantees minimum separation between entities, even as some cells fail. Once new failures cease occurring, in the case of a single target, the protocol is guaranteed to self-stabilize and the entities with feasible paths to the target cell make progress towards it. For multiple targets, failures may cause deadlocks in the system, so we identify a class of non-deadlocking failures where all entities are able to make progress to their respective targets. The algorithm relies on two general principles: temporary blocking for maintenance of safety and local geographical routing for guaranteeing progress. Our assertional proofs may serve as a template for the analysis of other distributed traffic control protocols. We present simulation results that provide estimates of throughput as a function of entity velocity, safety separation, single-target path complexity, failure-recovery rates, and multi-target path complexity.

==> prelim.tex <==
%\section{Preliminaries}
%\label{sec:prelim}
%

%\begin{definition}
%\label{def:tioa}
%A {\em Input/Output Automaton (IOA)\/} $\A$ is a tuple $(X,\Theta,A,\D)$ where
%%
%\begin{enumerate}[(a)]
%%
%\item $X$ is a set of state variables; $val(X)$ is the {\em state space\/}, 
%%
%\item $\Theta \subseteq val(X)$ is the set of {\em start states},
%%
%\item $A$ is a set of actions partitioned into input $I$, output $O$, and internal $H$ actions, and
%%
%\item ${\cal D} \subseteq val(X) \times A \times val(X)$ is a set of {\em transitions}.
%%
%A transition  $(\vx,a,\vx') \in \D$ is written as $\vx \sarrow{a}{\A} \vx'$ or as $\vx \arrow{a} \vx'$ when $\A$ is clear from the context.
%%
%\end{enumerate}
%\end{definition}
%%
%We denote the components of automata $\A$ by $X_\A$, $A_\A$, etc., and the components of automata $\A_i$ by $V_i$, $A_i$, etc. 
%
%An {\em execution fragment\/} of $\A$ is a finite or infinite sequence $\tau_0$ $a_1$ $\tau_1$ $a_2$ $\ldots$, such that for all $i$ in the sequence, $\tau_i.\lstate \arrow{a_{i+1}} \tau_{i+1}.\fstate$.
%%
%An execution fragment is an {\em execution\/} if $\tau_0.\fstate \in \Theta$.
%%
%The first state of $\alpha$, $\alpha.\fstate$, is $\tau_0.\fstate$, and for a closed $\alpha$, its last state, $\alpha.\lstate$, is the last state of its last trajectory.
%%
%The set of executions and reachable states of $\A$ are denoted by $\exec{\A}$ and $\reach{\A}$. 
%%
%A predicate $P$ is {\em stable \/} if for every pair of states $\vx$, $\vx^\prime \in val(X)$, $P(\vx)$ $\wedge$ $(\vx \arrow{a} \vx^\prime$ $\vee$ $\vx \arrow{\tau} \vx^\prime)$ implies $P(\vx^\prime)$.
%%
%{\em Invariant predicates\/} of $\A$ are those that contain $\reach{\A}$. 
%%
%A stable predicate $I$ is an {\em invariant\/} if for every start state $\vx \in \Theta$, $I(\vx)$ holds. 
%%

